Evaluation of Position-related Information in Multipath Components for Indoor Positioning

Location awareness is a key factor for a wealth of wireless indoor applications. Its provision requires the careful fusion of diverse information sources. For agents that use radio signals for localization, this information may either come from signal transmissions with respect to fixed anchors, from cooperative transmissions inbetween agents, or from radar-like monostatic transmissions. Using a-priori knowledge of a floor plan of the environment, specular multipath components can be exploited, based on a geometric-stochastic channel model. In this paper, a unified framework is presented for the quantification of this type of position-related information, using the concept of equivalent Fisher information. We derive analytical results for the Cram\'er-Rao lower bound of multipath-assisted positioning, considering bistatic transmissions between agents and fixed anchors, monostatic transmissions from agents, cooperative measurements inbetween agents, and combinations thereof, including the effect of clock offsets. Awareness of this information enables highly accurate and robust indoor positioning. Computational results show the applicability of the framework for the characterization of the localization capabilities of a given environment, quantifying the influence of different system setups, signal parameters, and the impact of path overlap.

==> CRLB_channel_apdx.tex <==
\subsubsection{Block Spectrum}

If we assume no path overlap (i.e. orthogonality) between signals from different VAs,  $\bLB = \bO$ and $\bLA$ is a
diagonal matrix. Using the resulting likelihood function (\ref{eq:sampledLHFortho}) derived in Appendix~\ref{app:lhf},
$\bLA$ can be rewritten as
%
\begin{align}\label{eq:FIM_LA} 
 [\bLA]_{\mpcidxsym,\mpcidxsym} & = 
  \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
  {\partial \tau\mpcidx \partial \tau\mpcidx}} \\
%
%  & = 2 \Re \left\{\alpha_k \alpha^*_{k}
%  \left(\frac{\partial \bs_{\tau\mpcidx}}{\partial \tau\mpcidx}\right)\Herm
%  \bC_\bn^{-1} \frac{\partial \bs_{\tau\mpcidx}}{\partial \tau\mpcidx}\right\} \\
%
  &= 2\Re \left\{ \frac{ |\alpha\mpcidx|^2 w\mpcidx^2 }{\sigman^2} \left(\frac{\partial \bs_{\tau\mpcidx}}{\partial
\tau\mpcidx}\right)\Herm \frac{\partial \bs_{\tau\mpcidx}}{\partial \tau\mpcidx} \right\} \nonumber \\
% 
  &= 2\Re \left\{ \frac{ |\alpha\mpcidx|^2w\mpcidx^2 }{\sigman^2} \frac{\partial^2}{\partial \tau\mpcidx^2}
   \sum_{i=1}^\timestepsymub s(i\Ts-\tau\mpcidx)s(i\Ts-\tau\mpcidx) \right\} \nonumber
\end{align}
%
Approximating the sum by an integral, we get
%
\begin{align*}
  [\bLA]_{\mpcidxsym,\mpcidxsym} &\approx 2 \Re \left\{ \frac{ |\alpha\mpcidx|^2 w\mpcidx^2  }{ \sigman^2}
\frac{\partial^2}{\partial \tau\mpcidx^2} \frac{1}{\Ts}\int_0^{\timestepsymub\Ts}
s(t-\tau\mpcidx)s(t-\tau\mpcidx)\mathrm{d}t \right\} \\
% 
  &= 2 \Re \left\{ \frac{ |\alpha\mpcidx|^2 w\mpcidx^2 }{ \sigman^2 \Ts} \int_f |2\pi f|^2 |S(f)|^2 \mathrm{d}f \right\}
\\
%
  &= \frac{8\pi^2\beta^2}{ N_0}|\alpha\mpcidx|^2 w\mpcidx^2
\end{align*}
where $\beta^2 = %\int_f f^2 |S(f)|^2 \mathrm{d}f/\int_f |S(f)|^2 \mathrm{d}f 
 \int_f f^2 |S(f)|^2 \mathrm{d}f$ is the effective (mean square) bandwidth for $s(t)$ normalized to unit energy.

\subsubsection{Non-Block Spectrum}

Using (\ref{eq:SS_LHFsampled_Freq}) derived in Appendix~\ref{app:lhf_NBS}, $\bLA$ can be rewritten as
%
\begin{align}
 [\bLA]_{\mpcidxsym,\mpcidxsym} & = 
  \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
  {\partial \tau\mpcidx \partial \tau\mpcidx}} \\
% 
  &= 8\pi|\alpha\mpcidx|^2 \int_f \frac{f^2|\mathrm{S}(f)|^2}{N_0 + S_\nu(\tau\mpcidx)|
  \mathrm{S}(f)|^2} \mathrm{d}f \nonumber \\
%
  &= \frac{8\pi}{N_0}|\alpha\mpcidx|^2w_k^2 \int_f f^2|\mathrm{S}(f)|^2 \frac{N_0 + \Tp S_\nu(\tau\mpcidx)}{N_0 +
S_\nu(\tau\mpcidx)| \mathrm{S}(f)|^2}\mathrm{d}f\nonumber \\
%
  &= \frac{8\pi\beta\mpcidx^2}{N_0}|\alpha\mpcidx|^2 w_k^2
\end{align}
where $\beta\mpcidx^2 = \int_f f^2|\mathrm{S}(f)|^2 \frac{N_0 + \Tp S_\nu(\tau\mpcidx)}{N_0 +
S_\nu(\tau\mpcidx)| \mathrm{S}(f)|^2}\mathrm{d}f$ represents the effective (mean square) bandwidth of the transmit pulse
$s(t)$ with applied whitening. As a result we can write
\begin{align}
  [\bLA]_{\mpcidxsym,\mpcidxsym} = 8\pi\beta^2 \frac{|\alpha\mpcidx|^2}{N_0 + \Tp S_\nu(\tau\mpcidx)}
  \frac{\beta\mpcidx^2}{\beta^2}
%
  = 8\pi\beta^2 \SINR\mpcidx \gamma\mpcidx.
\end{align}
where $\gamma\mpcidx$ is called bandwidth extension factor.
%
where $w\mpcidx^2 = N_0/(N_0 + \Tp S_\nu(\tau\mpcidx) )$ are DM weights of the orthogonal pulses, introducing an
effective (Nyquist) sampling period $\Tp$ that corresponds to a block spectrum approximating the pulse $s(t)$. 


% \begin{align}
%  [\bLA]_{\mpcidxsym,\mpcidxsym} & = 
%   \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
%   {\partial \tau\mpcidx \partial \tau\mpcidx}} \\
% % 
%   &=|\alpha|^2 \sum_{i=1}^\timestepsymub \frac{i^2|\mathrm{S}[i]|^2}{\sigman^2 + \Ts
%   S_\nu(\tau\mpcidx)|\mathrm{S}[i]|^2}\frac{8\pi}{N^2}
% \end{align}
% %
% Approximating the sum by an integral, we get
% %
% \begin{align}
%   [\bLA]_{\mpcidxsym,\mpcidxsym} & =8\pi|\alpha|^2 \int_f \frac{f^2|\mathrm{S}(f)|^2}{N_0 + S_\nu(\tau\mpcidx)|
%   \mathrm{S}(f)|^2} \mathrm{d}f \nonumber \\
% %
%   &= \frac{8\pi}{N_0}|\alpha|^2w_k^2 \int_f f^2|\mathrm{S}(f)|^2 \frac{N_0 + \Tp S_\nu(\tau\mpcidx)}{N_0 +
% S_\nu(\tau\mpcidx)| \mathrm{S}(f)|^2}\mathrm{d}f\nonumber \\
% %
%   &= \frac{8\pi\beta_w^2}{N_0}|\alpha|^2 w_k^2
% \end{align}
% where $\beta_w^2 = \int_f f^2|\mathrm{S}(f)|^2 \frac{N_0 + \Tp S_\nu(\tau\mpcidx)}{N_0 +
% S_\nu(\tau\mpcidx)| \mathrm{S}(f)|^2}\mathrm{d}f$ represents the effective (mean square) bandwidth of the transmit pulse
% $s(t)$ with applied whitening.

% We compute the FIM $\bJ_\bpsi$ of the auxiliary parameter vector $\bpsi = [\btau\T \ (\balpha\R)\T \ (\balpha\I)\T]\T$
% using (\ref{eq:sampledLHF}) and (\ref{eq:FIM_def}). We closely follow the notation of \cite{ShenTIT2010}. The FIM is
% decomposed according to the subvectors of $\bpsi$ into
% %
% \begin{equation}
%  \bJ_\bpsi = \left[ 
%  \begin{array}{lll}
%   \bLA & \bLB\R &\bLB\I \\
%   (\bLB\R)\T & \bLC' & \bO \\
%   (\bLB\I)\T & \bO & \bLC' 
%  \end{array}
%  \right] = \left[
%  \begin{array}{ll}
%  \bLA & \bLB \\
%  \bLB\T & \bLC
%  \end{array}
%  \right] .
% \end{equation}
% %
% Its elements are defined as
% 
% \begin{align*}
%  [\bLA]_{k,k'} & = 
% \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
% {\partial \tau_k \partial \tau_{k'}}} \\
% & = 2 \Re \left\{\alpha_k \alpha^*_{k'}
% \left(\frac{\partial \bs_{\tau_{k'}}}{\partial \tau_{k'}}\right)\Herm
% \bC_\bn^{-1} \frac{\partial \bs_{\tau_k}}{\partial \tau_k}\right\} \\
% %
%  [\bLB\R]_{k,k'} & = 
% \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
% {\partial \tau_k \partial \alpha_{k'}\R}} \\
% & = 2 \Re\left\{\alpha_k \left(\bs_{\tau_{k'}}\right)\Herm
% \bC_\bn^{-1} \frac{\partial \bs_{\tau_k}}{\partial \tau_k}\right\} \\
% %
%  [\bLB\I]_{k,k'} & = 
% \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
% {\partial \tau_k \partial \alpha_{k'}\I}} \\
% & = 2 \Im\left\{\alpha_k \left(\bs_{\tau_{k'}}\right)\Herm
% \bC_\bn^{-1} \frac{\partial \bs_{\tau_k}}{\partial \tau_k}\right\} \\
% %
%  [\bLC']_{k,k'} & = 
% \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
% {\partial \alpha_k\R \partial \alpha_{k'}\R}} 
% = 
% \E{\br|\bpsi}{ - \frac{\partial^2 \ln f(\br|\bpsi)}
% {\partial \alpha_k\I \partial \alpha_{k'}\I}} \\
% & = 2 \Re\left\{ \left(\bs_{\tau_{k}}\right)\Herm
% \bC_\bn^{-1} \bs_{\tau_{k'}}\right\} \\
% \end{align*}
% %
% where $\bs_{\tau_k}= \begin{bmatrix} s(T_s-\tau_k) & \ldots & s(\timestepsymub T_s-\tau_k) \end{bmatrix}\Herm$. 

==> pst-sigsys.tex <==
%%
%% This is file `pst-sigsys.tex' v 1.4.
%%
%% IMPORTANT NOTICE:
%%
%% (C)
%% Farshid Delgosha (NY - U.S.A.) <fdelgosha@gmail.com>
%%
%% v 1.0: 01/15/2009
%% v 1.1: 04/01/2009
%% v 1.2: 01/15/2010
%% v 1.3: 06/18/2010
%% v 1.4: 03/07/2011
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN archives
%% in directory macros/latex/base/lppl.txt.
%%
%% DESCRIPTION:
%%   `pst-sigsys' is a PSTricks package for drawing block diagrams
%%    related to the signal processing discipline.
%%
%
\csname PSTsigsysLoaded\endcsname
\let\PSTsigsysLoaded\endinput

\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTnodesLoaded\endinput\else\input pst-node.tex\fi
\ifx\PSTXKeyLoaded\endinput\else \input pst-xkey \fi

\def\pstsigsysFV{1.4}
\def\pstsigsysFD{2011/03/07}
\message{`PST-SigSys' v\pstsigsysFV, \pstsigsysFD\space (fd)}


\SpecialCoor



%--- new pstricks styles ---------------------------------
\newpsstyle{ArrowLen}{arrowsize=1.35mm,arrowlength=1.25,arrowinset=.25}
\newpsstyle{Arrow}{arrows=->,style=ArrowLen}
\newpsstyle{Dash}{linestyle=dashed,dash=.15 .08}
\newpsstyle{Graph}{linewidth=1.25pt,linearc=0}
\newpsstyle{Stem}{linewidth=1.25pt,linestyle=solid,stemhead=*}
\newpsstyle{RoundCorners}{framesep=.125,framearc=.25,linearc=.1}
%--- end new pstricks styles -----------------------------


%--- new pstricks-add styles -----------------------------
\AtBeginDocument{
\ifx\PSTricksAddLoaded\endinput
\newpsstyle{ArrowIn}{ArrowInside=->,style=ArrowLen}
\newpsstyle{DashDot}{linestyle=dashed,dash=.15 .055 .04 .055}
\newpsstyle{Brace}{braceWidth=.02,braceWidthInner=.115,braceWidthOuter=.115,ref=C}
\newpsobject{psBraceUp}{psbrace}{style=Brace,rot=-90,nodesepB=-\pslabelsep}
\newpsobject{psBraceDown}{psbrace}{style=Brace,rot=90,nodesepB=\pslabelsep}
\newpsobject{psBraceRight}{psbrace}{style=Brace,rot=-90,nodesepA=\pslabelsep}
\newpsobject{psBraceLeft}{psbrace}{style=Brace,rot=-90,nodesepA=-\pslabelsep}
\fi
}
%--- end new pstricks-add styles -------------------------


%--- internal macros -------------------------------------
\newdimen\ss@ticklength
\newdimen\ss@signalsep
\newdimen\ss@zerowidth
\newdimen\ss@zeroradius
\newdimen\ss@zeroradiusinc
\newdimen\ss@polewidth
\newdimen\ss@polelength
\newdimen\ss@oplength
\newdimen\ss@opwidth
\newdimen\ss@opsep
\newdimen\ss@ldotssep
\newdimen\ss@ldotssize
\newdimen\ss@aoffset
\newdimen\ss@knoblength
\newdimen\ss@knobwidth
\def\ss@knobangle{}
%
\newdimen\ss@temp@dimA
\newdimen\ss@temp@dimB
\newdimen\ss@temp@dimC
\newcount\ss@temp@cnt
\def\ss@temp{}
\def\ss@temp@choice{}
%
%%% add two numbers %%%
\newdimen\ss@calc@dim
\def\ss@calc{}
\def\ss@addnum#1#2#3{%
\ss@calc@dim=#1pt%
\advance\ss@calc@dim #2pt%
\pst@divide{\ss@calc@dim}{1pt}\ss@calc%
\let#3\ss@calc%
}
%
\def\pst@scale#1{\pssetlength{#1}{\ss@scale#1}}
%
%%% draw a cross %%%
\def\ss@cross@temp{}
\def\pst@cross(#1;#2)#3{%
\ss@addnum{#2}{90}\ss@cross@temp%
\psline[linewidth=#3,arrows=-](-#1;#2)(#1;#2)%
\psline[linewidth=#3,arrows=-](-#1;\ss@cross@temp)(#1;\ss@cross@temp)%
}
%
%%% set frame width %%%
\def\pst@frame@width#1{%
\pssetlength{\ss@temp@dimA}{#1}%
\divide\ss@temp@dimA 2\relax%
\edef\psk@framewidth{\pst@number\ss@temp@dimA}%
}
%
%%% set frame height %%%
\def\pst@frame@height#1{%
\pssetlength{\ss@temp@dimA}{#1}%
\divide\ss@temp@dimA 2\relax%
\edef\psk@frameheight{\pst@number\ss@temp@dimA}%
}
%
%%% set the frame width using the golden ratio %%%
\def\pst@gratio@width#1#2{%
\pssetlength{\ss@temp@dimA}{#1}%
\pssetlength{\ss@temp@dimB}{#2\ss@temp@dimA}%
\divide\ss@temp@dimA 2\relax%
\divide\ss@temp@dimB 2\relax%
\edef\psk@framewidth{\pst@number\ss@temp@dimA}%
\edef\psk@frameheight{\pst@number\ss@temp@dimB}%
}
%
%%% set the frame height using the golden ratio %%%
\def\pst@gratio@height#1#2{%
\pssetlength{\ss@temp@dimA}{#1}%
\pssetlength{\ss@temp@dimB}{#2\ss@temp@dimA}%
\divide\ss@temp@dimA 2\relax%
\divide\ss@temp@dimB 2\relax%
\edef\psk@frameheight{\pst@number\ss@temp@dimA}%
\edef\psk@framewidth{\pst@number\ss@temp@dimB}%
}
%
\newpsstyle{inv@frame}{fillstyle=none,linestyle=none,framearc=0}
%
%%% ss@ifneqdim %%%
\newdimen\ss@if@dimA
\newdimen\ss@if@dimB
\def\ss@ifneqdim#1#2#3{%
\pssetlength{\ss@if@dimA}{#1}%
\pssetlength{\ss@if@dimB}{#2}%
\ifdim\ss@if@dimA=\ss@if@dimB\else%
#3\fi}
%
%%% This is my parser. %%%
\def\ss@parse@temp{}
\def\ss@parseA{}
\def\ss@parseB{}
\def\ss@parseC{}
%
\def\ss@parse@III#1{%
\ss@parse@II{#1}{\ss@parseA}{\ss@parse@temp}%
\ss@parse@II{\ss@parse@temp}{\ss@parseB}{\ss@parseC}%
}
%
\def\ss@parse@II#1#2#3{\expandafter\ss@parse#1 \@nil#2#3}
%
\def\ss@parse#1 #2\@nil#3#4{%
\gdef#3{#1}%
\ifx\@empty#2\@empty%
\gdef#4{}%
\else%
\ss@removespace#2\@nil#4%
\fi%
}
%
\def\ss@removespace#1 \@nil#2{\gdef#2{#1}}
%--- end internal macros ---------------------------------


%--- keys ------------------------------------------------
\define@key[psset]{pst-sigsys}{scale}{\def\ss@scale{#1}}
\define@choicekey*[psset]{pst-sigsys}{xlpos}[\val\ss@temp@choice]{b,t}{%
\ifcase\ss@temp@choice\relax%
\def\ss@xlpos{b}%
\or%
\def\ss@xlpos{t}%
\fi%
}
\define@choicekey*[psset]{pst-sigsys}{ylpos}[\val\ss@temp@choice]{r,l}{%
\ifcase\ss@temp@choice\relax%
\def\ss@ylpos{r}%
\or%
\def\ss@ylpos{l}%
\fi%
}
\define@key[psset]{pst-sigsys}{ticklength}{\pssetlength{\ss@ticklength}{#1}}
\define@key[psset]{pst-sigsys}{signalsep}{\pssetlength{\ss@signalsep}{#1}}
\define@key[psset]{pst-sigsys}{stemhead}[]{\def\ss@stemhead{#1}}
\define@boolkey[psset]{pst-sigsys}[ss@]{stemtag}[true]{}
\define@key[psset]{pst-sigsys}{stemtagformat}[]{\def\ss@stemtagformat{#1}}
\define@boolkey[psset]{pst-sigsys}[ss@]{killzero}[true]{}
\define@key[psset]{pst-sigsys}{order}{\def\ss@order{#1}}
\define@key[psset]{pst-sigsys}{zerowidth}{\pssetlength{\ss@zerowidth}{#1}}
\define@key[psset]{pst-sigsys}{zeroradius}{\pssetlength{\ss@zeroradius}{#1}}
\define@key[psset]{pst-sigsys}{zeroradiusinc}{\pssetlength{\ss@zeroradiusinc}{#1}}
\define@key[psset]{pst-sigsys}{polewidth}{\pssetlength{\ss@polewidth}{#1}}
\define@key[psset]{pst-sigsys}{polelength}{\pssetlength{\ss@polelength}{#1}}
\define@key[psset]{pst-sigsys}{opwidth}{\pssetlength{\ss@opwidth}{#1}}
\define@key[psset]{pst-sigsys}{oplength}{\pssetlength{\ss@oplength}{#1}}
\define@key[psset]{pst-sigsys}{opsep}{\pssetlength{\ss@opsep}{#1}}
\define@choicekey*[psset]{pst-sigsys}{operation}[\val\ss@temp@choice]{plus,times}{%
\ifcase\ss@temp@choice\relax%
\def\ss@angle{0}%
\or%
\def\ss@angle{45}%
\fi%
}
\define@key[psset]{pst-sigsys}{angle}{\def\ss@angle{#1}}
\define@key[psset]{pst-sigsys}{ldotssize}{\pssetlength{\ss@ldotssize}{#1}}
\define@key[psset]{pst-sigsys}{ldotssep}{\pssetlength{\ss@ldotssep}{#1}}
\define@key[psset]{pst-sigsys}{gratioWh}{\pst@gratio@width{#1}{.6180339887}}
\define@key[psset]{pst-sigsys}{gratioWv}{\pst@gratio@width{#1}{1.618033989}}
\define@key[psset]{pst-sigsys}{gratioHh}{\pst@gratio@height{#1}{1.618033989}}
\define@key[psset]{pst-sigsys}{gratioHv}{\pst@gratio@height{#1}{.6180339887}}
\define@key[psset]{pst-sigsys}{aoffset}{\pssetlength{\ss@aoffset}{#1}}
\define@key[psset]{pst-sigsys}{afac}{\def\ss@afac{#1}}
\define@key[psset]{pst-sigsys}{knoblength}{\pssetlength{\ss@knoblength}{#1}}
\define@key[psset]{pst-sigsys}{knobwidth}{\pssetlength{\ss@knobwidth}{#1}}
\define@key[psset]{pst-sigsys}{knobangle}{\def\ss@knobangle{#1}}

\define@key[psset]{pst-sigsys}{framewidth}{\pst@frame@width{#1}}
\define@key[psset]{pst-sigsys}{frameheight}{\pst@frame@height{#1}}
\define@key[psset]{pst-sigsys}{FillColor}{\psset{fillstyle=solid,fillcolor=#1}}
%--- end keys --------------------------------------------


%--- default key values ----------------------------------
\psset[pst-sigsys]{scale=1,angle=0}%  global
\psset[pst-sigsys]{xlpos=b,ylpos=r}%  psaxeslabels
\psset[pst-sigsys]{ticklength=.15}%  psTick
\psset[pst-sigsys]{signalsep=5pt}%  pssignal
\psset[pst-sigsys]{stemhead=*,stemtag=false,stemtagformat=\scriptstyle,killzero=false}%  psstem
\psset[pst-sigsys]{zerowidth=.7pt,zeroradius=.08,zeroradiusinc=.07,order=1}%  pszero
\psset[pst-sigsys]{polewidth=.7pt,polelength=.12}%  pspole
\psset[pst-sigsys]{opwidth=.7pt,oplength=.125,opsep=.1,operation=plus}%  pscircleop and psframeop
\psset[pst-sigsys]{ldotssize=.05,ldotssep=.15}%  psldots
\psset[pst-sigsys]{aoffset=0,afac=1}%  psadaptive
\psset[pst-sigsys]{knobwidth=.7pt,knoblength=1,knobangle=45}%  psknob
%--- end default key values ------------------------------

\pst@addfams{pst-sigsys}


%--- psaxeslabels ----------------------------------------
\def\psaxeslabels{\def\pst@par{}\pst@object{psaxeslabels}}
\def\psaxeslabels@i{\pst@getarrows\psaxeslabels@ii}
\def\psaxeslabels@ii(#1,#2)(#3,#4)(#5,#6)#7#8{{%
\use@par%
\ss@ifneqdim{#3}{#5}{\psline(#3,#2)(#5,#2)}%
\ss@ifneqdim{#4}{#6}{\psline(#1,#4)(#1,#6)}%
%
\if\ss@xlpos t%
\rput(#5,#2){\rput[rb](0,\pslabelsep){#7}}%
\else%
\rput(#5,#2){\rput[rt](0,-\pslabelsep){#7}}%
\fi%
%
\if\ss@ylpos l%
\rput(#1,#6){\rput[tr](-\pslabelsep,0){#8}}%
\else%
\rput(#1,#6){\rput[tl](\pslabelsep,0){#8}}%
\fi%
}\ignorespaces}
%--- end psaxeslabels ------------------------------------


%--- pstick ----------------------------------------------
\def\pstick{\def\pst@par{}\pst@object{pstick}}
\def\pstick@i{\@ifnextchar({\pstick@ii{\ss@angle}}{\pstick@ii}}
\def\pstick@ii#1(#2)#3{{%
\use@par%
\pssetlength{\ss@temp@dimA}{#3}%
\pssetlength{\ss@temp@dimA}{.5\ss@temp@dimA}%
\rput(#2){\psline(-\ss@temp@dimA;#1)(\ss@temp@dimA;#1)}%
}\ignorespaces}
%--- end pstick ------------------------------------------


%--- psTick ----------------------------------------------
\def\psTick{\def\pst@par{}\pst@object{psTick}}
\def\psTick@i{\@ifnextchar({\psTick@ii{\ss@angle}}{\psTick@ii}}
\def\psTick@ii#1(#2){{%
\use@par%
\pstick@ii#1(#2){\ss@ticklength}%
}\ignorespaces}
%--- end psTick ------------------------------------------


%--- pssignal --------------------------------------------
\def\pssignal{\def\pst@par{}\pst@object{pssignal}}
\def\pssignal@i(#1)#2#3{{%
\use@par%
\rput(#1){\rnode{#2}{\psframebox[style=inv@frame,framesep=\ss@signalsep]{#3}}}%
}\ignorespaces}
%--- end pssignal ----------------------------------------


%--- psstem ----------------------------------------------
\def\psstem{\def\pst@par{}\pst@object{psstem}}
\def\psstem@i{\@ifnextchar({\psstem@ii}{\psstem@ii(0,1)}}
\def\psstem@ii(#1,#2)#3{{%
\use@par%
\ss@temp@cnt=#1%
\@for\ss@for@ind:=#3\do{%
\pssetlength{\ss@temp@dimA}{\ss@for@ind}%
\ifss@killzero%
\ifdim\ss@temp@dimA=\z@\else%
\psline{-\ss@stemhead}(\ss@temp@cnt,0)(\ss@temp@cnt,\ss@for@ind)%
\fi\else%
\psline{-\ss@stemhead}(\ss@temp@cnt,0)(\ss@temp@cnt,\ss@for@ind)%
\fi%
%
\ifss@stemtag%
\ifdim\ss@temp@dimA<\z@%
\rput[b](\ss@temp@cnt,\pslabelsep){$\ss@stemtagformat\the\ss@temp@cnt$}%
\else%
\rput[t](\ss@temp@cnt,-\pslabelsep){$\ss@stemtagformat\the\ss@temp@cnt$}%
\fi\fi%
%
\advance\ss@temp@cnt#2}%
}\ignorespaces}
%--- end psstem ------------------------------------------


%--- pszero ----------------------------------------------
\def\pszero{\def\pst@par{}\pst@object{pszero}}
\def\pszero@i(#1)#2{{%
\use@par%
\pst@scale{\ss@zerowidth}%
\pst@scale{\ss@zeroradius}%
\pst@scale{\ss@zeroradiusinc}%
\pssetlength{\ss@temp@dimA}{\ss@zeroradius}%
\ss@temp@cnt=\ss@order%
\loop%
\cnode[linewidth=\ss@zerowidth](#1){\ss@temp@dimA}{#2}%
\psaddtolength{\ss@temp@dimA}{\ss@zeroradiusinc}%
\ifnum\ss@temp@cnt>\@ne%
\advance\ss@temp@cnt-\@ne%
\repeat%
}\ignorespaces}
%--- end pszero ------------------------------------------


%--- pspole ----------------------------------------------
% The main part of this code is borrowed from pst-node
%
\def\pspole{\def\pst@par{}\pst@object{pspole}}
\def\pspole@i(#1)#2{%
\leavevmode%
\hbox{%
\use@par%
\pst@scale{\ss@polelength}%
\pst@scale{\ss@polewidth}%
\pst@@getcoor{#1}%
\pssetlength\pst@dimc{\ss@polelength}%
\pst@dimg=\psk@dimen\pslinewidth%
\advance\pst@dimc-\pst@dimg%
\advance\pst@dimc.5\pslinewidth%
\ifPst@nodealign%
\kern\pst@dimc%
\vrule width\z@ height \pst@dimc depth \pst@dimc%
\fi%
\rput(#1){\pst@cross(\ss@polelength;45){\ss@polewidth}}%
\pst@newnode{#2}{11}{\pst@coor \pst@number\pst@dimc}{\tx@InitCnode}%
\ifPst@nodealign\kern\pst@dimc\fi%
}\ignorespaces}
%--- end pspole ------------------------------------------


%--- pscircleop ------------------------------------------
\def\pscircleop{\def\pst@par{}\pst@object{pscircleop}}
\def\pscircleop@i(#1)#2{{%
\use@par%
\pst@scale{\ss@oplength}%
\pst@scale{\ss@opsep}%
\pst@scale{\ss@opwidth}%
\pst@scale{\pslinewidth}%
\pssetlength{\ss@temp@dimA}{\ss@oplength}%
\psaddtolength{\ss@temp@dimA}{\ss@opsep}%
\cnode(#1){\ss@temp@dimA}{#2}%
\rput(#1){\pst@cross(\ss@oplength;\ss@angle){\ss@opwidth}}%
}\ignorespaces}
%--- end pscircleop --------------------------------------


%--- psframeop -------------------------------------------
\def\psframeop{\def\pst@par{}\pst@object{psframeop}}
\def\psframeop@i(#1)#2{{%
\use@par%
\pst@scale{\ss@oplength}%
\pst@scale{\ss@opsep}%
\pst@scale{\ss@opwidth}%
\pst@scale{\pslinewidth}%
\pssetlength{\ss@temp@dimA}{2\ss@oplength}%
\psaddtolength{\ss@temp@dimA}{2\ss@opsep}%
\fnode[framesize=\ss@temp@dimA](#1){#2}%
\rput(#1){\pst@cross(\ss@oplength;\ss@angle){\ss@opwidth}}%
}\ignorespaces}
%--- end psframeop ---------------------------------------


%--- psdisk ----------------------------------------------
\def\psdisk{\def\pst@par{}\pst@object{psdisk}}
\def\psdisk@i(#1)#2{{%
\use@par%
\pscircle*[linestyle=none,linecolor=\psfillcolor](#1){#2}%
}\ignorespaces}
%--- end psdisk ------------------------------------------


%--- psring ----------------------------------------------
\def\psring{\def\pst@par{}\pst@object{psring}}
\def\psring@i(#1)#2#3{{%
\use@par%
\pssetlength{\ss@temp@dimA}{#2}%
\pssetlength{\ss@temp@dimB}{#3}%
\psaddtolength{\ss@temp@dimB}{-\ss@temp@dimA}%
\pscircle[dimen=inner,linewidth=\ss@temp@dimB,linecolor=\psfillcolor](#1){\ss@temp@dimA}%
}\ignorespaces}
%--- end psring ------------------------------------------


%--- psdiskc ---------------------------------------------
\def\psdiskc{\def\pst@par{}\pst@object{psdiskc}}
\def\psdiskc@i(#1)(#2,#3)#4{{%
\use@par%
\pssetlength{\ss@temp@dimA}{#2}%
\pssetlength{\ss@temp@dimB}{#3}%
\ifdim\ss@temp@dimA>\ss@temp@dimB%
\pssetlength{\ss@temp@dimC}{1.5\ss@temp@dimA}%
\else%
\pssetlength{\ss@temp@dimC}{1.5\ss@temp@dimB}%
\fi%
\psclip{\rput(#1){\psframe[linestyle=none,linecolor=\psfillcolor](-#2,-#3)(#2,#3)}}%
\psring@i(#1){#4}{\ss@temp@dimC}%
\endpsclip%
}\ignorespaces}
%--- end psdiskc -----------------------------------------


%--- psldots ---------------------------------------------
\def\psldots{\def\pst@par{}\pst@object{psldots}}
\def\psldots@i{\@ifnextchar({\psldots@ii{\ss@angle}}{\psldots@ii}}
\def\psldots@ii#1(#2){{%
\use@par%
\pst@scale{\ss@ldotssep}%
\pst@scale{\ss@ldotssize}%
\rput(#2){\psdots[dotsize=\ss@ldotssize](-\ss@ldotssep;#1)(0,0)(\ss@ldotssep;#1)}%
}\ignorespaces}
%--- end psldots -----------------------------------------


%--- ldotsnode -------------------------------------------
\def\ldotsnode{\def\pst@par{}\pst@object{ldotsnode}}
\def\ldotsnode@i{\@ifnextchar({\ldotsnode@ii{\ss@angle}}{\ldotsnode@ii}}
\def\ldotsnode@ii#1(#2)#3{{%
\use@par%
\ss@temp@dimC=.5\ss@signalsep%
\ss@temp@dimB=.5\ss@ldotssize%
\advance\ss@temp@dimB\ss@temp@dimC%
\ss@temp@dimA=\ss@ldotssep%
\advance\ss@temp@dimA\ss@temp@dimB%
\advance\ss@temp@dimA\ss@temp@dimC%
\edef\psk@framewidth{\pst@number\ss@temp@dimA}%
\edef\psk@frameheight{\pst@number\ss@temp@dimB}%
\rput{#1}(#2){\fnode[style=inv@frame](0,0){#3}}%
\psldots{#1}(#2)%
}\ignorespaces}
%--- end ldotsnode ---------------------------------------


%--- psblock ---------------------------------------------
\def\psblock{\def\pst@par{}\pst@object{psblock}}
\def\psblock@i(#1)#2#3{{%
\use@par%
\rput(#1){\rnode{#2}{\psframebox{#3}}}%
}\ignorespaces}
%--- end psblock -----------------------------------------


%--- psfblock --------------------------------------------
\def\psfblock{\def\pst@par{}\pst@object{psfblock}}
\def\psfblock@i(#1)#2#3{{%
\use@par%
\fnode(#1){#2}%
\rput(#1){#3}%
}\ignorespaces}
%--- end psfblock ----------------------------------------


%--- psadaptive ------------------------------------------
\def\psadaptive{\def\pst@par{}\pst@object{psadaptive}}
\def\psadaptive@i{\check@arrow{\psadaptive@ii}}
\def\psadaptive@ii#1(#2)#3{{%
\use@par%
\nodexn{(#1)+(#2)}{ss@nodeA}%
\nodexn{(ss@nodeA)+(\ss@aoffset,0)}{#3}%
\psLNode(#1)(ss@nodeA){-\ss@afac}{ss@nodeB}%
\ifdim\ss@aoffset>\z@%
\ncdiagg[armA=\ss@aoffset,angleA=180]{-}{#3}{#1}%
\else%
\ncdiagg[armA=-\ss@aoffset,angleA=0]{-}{#3}{#1}%
\fi%
\ncline{#1}{ss@nodeB}%
}\ignorespaces}
%--- end psadaptive --------------------------------------


%--- psknob ----------------------------------------------
\def\psknob{\def\pst@par{}\pst@object{psknob}}
\def\psknob@i(#1)#2{{%
\psset{arrows=->}%
\use@par%
\pst@scale{\ss@knobwidth}%
\pst@scale{\ss@knoblength}%
\pssetlength{\ss@temp@dimA}{\psk@radius}%
\pst@scale{\ss@temp@dimA}%
\cnode[linewidth=\ss@knobwidth](#1){\ss@temp@dimA}{#2}%
\pstick[linewidth=\ss@knobwidth]{\ss@knobangle}(#1){\ss@knoblength}%
}\ignorespaces}
%--- end psknob ------------------------------------------


%--- psusampler ------------------------------------------
\def\psusampler{\def\pst@par{}\pst@object{psusampler}}
\def\psusampler@i(#1)#2#3{{%
\use@par%
\psfblock(#1){#2}{$\mathord{\uparrow}#3$}%
}\ignorespaces}
%--- end psusampler --------------------------------------


%--- psdsampler ------------------------------------------
\def\psdsampler{\def\pst@par{}\pst@object{psdsampler}}
\def\psdsampler@i(#1)#2#3{{%
\use@par%
\psfblock(#1){#2}{$\mathord{\downarrow}#3$}%
}\ignorespaces}
%--- end psdsampler --------------------------------------


%--- nclist ----------------------------------------------
\def\nclist{\def\pst@par{}\pst@object{nclist}}
\def\nclist@i{\check@arrow{\nclist@ii}}
\def\nclist@ii#1{\@ifnextchar[{\nclist@iii{#1}}{\nclist@iv{#1}}}
%
\def\nclist@iii#1[#2]#3{{%
\use@par%
\def\ss@prevnode{}%
\@for\ss@for@ind:=#3\do{%
\ifx\@empty\ss@prevnode\@empty%
\let\ss@prevnode\ss@for@ind%
\else%
\ss@parse@III{\ss@for@ind}%
\csname#1\endcsname{\ss@prevnode}{\ss@parseA}%
\ifx\@empty\ss@parseB\@empty\else%
\ifx\@empty\ss@parseC\@empty%
\csname#2\endcsname{\ss@parseB}%
\else%
\csname\ss@parseB\endcsname{\ss@parseC}%
\fi\fi%
\let\ss@prevnode\ss@parseA%
\fi%
}%
}\ignorespaces}
%
\def\nclist@iv#1#2{{%
\use@par%
\def\ss@prevnode{}%
\@for\ss@for@ind:=#2\do{%
\ifx\@empty\ss@prevnode\@empty%
\else%
\csname#1\endcsname{\ss@prevnode}{\ss@for@ind}%
\fi%
\let\ss@prevnode\ss@for@ind%
}%
}\ignorespaces}
%--- end nclist ------------------------------------------


%--- ncstar ----------------------------------------------
\def\ncstar{\def\pst@par{}\pst@object{ncstar}}
\def\ncstar@i{\check@arrow{\ncstar@ii}}
\def\ncstar@ii#1{\@ifnextchar[{\ncstar@iii{#1}}{\ncstar@iv{#1}}}
%
\def\ncstar@iii#1[#2]#3#4{{%
\use@par%
\@for\ss@for@ind:=#3\do{%
\ss@parse@III{\ss@for@ind}%
\csname#1\endcsname{\ss@parseA}{#4}%
\ifx\@empty\ss@parseB\@empty\else%
\ifx\@empty\ss@parseC\@empty%
\csname#2\endcsname{\ss@parseB}%
\else%
\csname\ss@parseB\endcsname{\ss@parseC}%
\fi\fi%
}%
}\ignorespaces}
%
\def\ncstar@iv#1#2#3{{%
\use@par%
\@for\ss@for@ind:=#2\do{\csname#1\endcsname{\ss@for@ind}{#3}}%
}\ignorespaces}
%--- end ncstar ------------------------------------------
\endinput 
